Multilingual and Fully Non-Autoregressive ASR with Large Language Model Fusion: A Comprehensive Study

In the era of large models, the autoregressive nature of decoding often results in latency serving as a significant bottleneck. We propose a non-autoregressive LM-fused ASR system that effectively leverages the parallelization capabilities of accelerator hardware. Our approach combines the Universal Speech Model (USM) and the PaLM 2 language model in per-segment scoring mode, achieving an average relative WER improvement across all languages of 10.8% on FLEURS and 3.6% on YouTube captioning. Furthermore, our comprehensive ablation study analyzes key parameters such as LLM size, context length, vocabulary size, fusion methodology. For instance, we explore the impact of LLM size ranging from 128M to 340B parameters on ASR performance. This study provides valuable insights into the factors influencing the effectiveness of practical large-scale LM-fused speech recognition systems.

==> intro_and_related_work.tex <==
% Focus more on multilinguality?

\section{Introduction}

Large-scale language model (LLM) have become increasingly popular in recent years due to their ability to understand human language, generate human-like text, and complete a wide range of tasks. Trained on gigantic amounts of text data, LLM families such as GPT, PaLM, LLaMA have shown state-of-the-art results across several natural language processing (NLP) and search tasks including chatbot, machine translation and many zero-shot or few-shot learning applications. There are also increasing interest in applying these LLMs in Automated Speech Recognition (ASR).
% Can we still say that???
% However, the applications of these LLMs in Automated Speech Recognition (ASR) still remain limited.
There are also increasing interest in applying these LLMs in Automated Speech Recognition (ASR).

Recent 

In this paper, we

\section{Related Works}

Several approaches of applying LMs to end-to-end ASR models have been discussed in the literature. Rescoring takes the hypotheses generated by the ASR model and then scores them again using an LM. Fusion strategies such as \textit{shallow}~\cite{peyser2020improving}, \textit{cold}~\cite{sriram2017cold}, \textit{deep}~\cite{gulcehre2015using} and \textit{component}~\cite{shan2019component} fusion allow the scores from LMs employed during the decoding stage~\cite{hori2014real, chorowski2016towards, hori2018end}. However, for large scale ASR, there have been relatively small gains from incorporating LMs in these fashions ~\cite{kannan2018analysis}. 
